A Panda? No, It's a Sloth: Slowdown Attacks on Adaptive Multi-Exit Neural Network Inference

Recent increases in the computational demands of deep neural networks (DNNs), combined with the observation that most input samples require only simple models, have sparked interest in $input$-$adaptive$ multi-exit architectures, such as MSDNets or Shallow-Deep Networks. These architectures enable faster inferences and could bring DNNs to low-power devices, e.g., in the Internet of Things (IoT). However, it is unknown if the computational savings provided by this approach are robust against adversarial pressure. In particular, an adversary may aim to slowdown adaptive DNNs by increasing their average inference time$-$a threat analogous to the $denial$-$of$-$service$ attacks from the Internet. In this paper, we conduct a systematic evaluation of this threat by experimenting with three generic multi-exit DNNs (based on VGG16, MobileNet, and ResNet56) and a custom multi-exit architecture, on two popular image classification benchmarks (CIFAR-10 and Tiny ImageNet). To this end, we show that adversarial example-crafting techniques can be modified to cause slowdown, and we propose a metric for comparing their impact on different architectures. We show that a slowdown attack reduces the efficacy of multi-exit DNNs by 90-100%, and it amplifies the latency by 1.5-5$\times$ in a typical IoT deployment. We also show that it is possible to craft universal, reusable perturbations and that the attack can be effective in realistic black-box scenarios, where the attacker has limited knowledge about the victim. Finally, we show that adversarial training provides limited protection against slowdowns. These results suggest that further research is needed for defending multi-exit architectures against this emerging threat. Our code is available at https://github.com/sanghyun-hong/deepsloth.

==> impact.tex <==

% : Mandatory
\section*{Broader Impact}
%
Over the last few years, deep learning workloads have seen a rapid increase in their resource consumption; for example, training GPT-2 language models has a carbon footprint equivalent to a total of six cars in their lifetime~\cite{Energy:Strubell}.
%
The Input-adaptive inference techniques are a promising direction for reducing the footprint of the post-training operations of these workloads.
%
Our work shows that an adversary can negate this reduction and cause operational challenges for deep learning practitioners.
%
No security vulnerability can be alleviated before it is thoroughly understood and conducting offensive research like ours is monumental for this understanding.
%
Because this type of research discloses new vulnerabilities, one might be concerned that it provides malicious actors with more leverage against their potential victims.
%
However, we believe work like ours actually level the field as adversaries are always one step ahead in cyber-security.
%
Finally, as deep learning finds its way into an oppressor's toolbox, in the forms of mass surveillance~\cite{Feldstein:Repression}
or racial profiling~\cite{Ethnicity:Wang}; by studying its weaknesses our best hope is to provide its potential victims means of self-protection.

==> motivation.tex <==
This observation applies to even to standard, non-adaptive, DNNs that process all input samples identically.
%
As a case study, we use the Shallow-Deep Network (SDN) modification~\cite{SDN:Kaya} to convert three standard convolutional neural networks (CNNs) into adaptive multi-exit models.
%
The resulting models produce a sequence of classifications, i.e., \emph{early-exits}, from their internal classifiers at each hidden convolutional block.
%
The early-exit capability (EEC) plots in Figure~\ref{fig:oracle_early_exits} indicate the fraction of the test-time samples that exit early at a specific fraction of the model's full inference cost.
%
For example, a VGG-16 model can correctly classify $\sim$50\% of the samples in the Tiny ImageNet task when it uses only $\sim$50\% of its full cost.


\input{figures/motivation_images.tex}

To demonstrate what makes a sample easy-to-detect, Figure~\ref{fig:simple_complex} presents a selection of test images from Tiny ImageNet that early-exit at different blocks of the VGG16. 
%
The easy samples that require less computation are more typical and, therefore, have more support from the training set.
%
Note that here we unrealistically assume that the computation stops as soon as a hidden block correctly classifies the sample.
%
In Sec~\ref{sec:our-attack}, we will discuss the practical ways of stopping the computation.


We define the \emph{lateness} of a multi-exit model as ($1$ - AUC), where AUC is the area under its EEC curve---estimated via the trapezoidal rule.
%
The closer the lateness is to $1$, the less capable a model is of using its early-exits on the input samples.
%
In our paper, we utilize the generic SDN modification to study the robustness of multi-exit models to adversaries who, by perturbing the input samples, wish to increase a victim model's lateness.
%
Such adversaries threaten the safety of DNNs as lateness is a measure of a model's inference cost and time.


==> problem.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% problem.tex  --
%  
%   Problem statement, goals, non-goals.
%
% !TEX root = main.tex
% Last modified:		$Date:: 2020-04-10 #$  by   $Author: shhong $
% SVN revision:   	$Rev: 7938 $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Problem statement}
\label{sec:problem}

